Painless Federated Learning: An Interplay of Line-Search and Extrapolation

The classical line search for learning rate (LR) tuning in the stochastic gradient descent (SGD) algorithm can tame the convergence slowdown due to data-sampling noise. In a federated setting, wherein the client heterogeneity introduces a slowdown to the global convergence, line search can be relevantly adapted. In this work, we show that a stochastic variant of line search tames the heterogeneity in federated optimization in addition to that due to client-local gradient noise. To this end, we introduce Federated Stochastic Line Search (FedSLS) algorithm and show that it achieves deterministic rates in expectation. Specifically, FedSLS offers linear convergence for strongly convex objectives even with partial client participation. Recently, the extrapolation of the server's LR has shown promise for improved empirical performance for federated learning. To benefit from extrapolation, we extend FedSLS to Federated Extrapolated Stochastic Line Search (FedExpSLS) and prove its convergence. Our extensive empirical results show that the proposed methods perform at par or better than the popular federated learning algorithms across many convex and non-convex problems.

==> sections/discuss.tex <==
This paper presents a framework \fli for federated learning where clients communicate the step-size and local objective values in addition to the model at every synchronization round. The communicated values are synchronized alongside the model and used to efficiently scale global model updates. An interesting result presented in this work shows that if the local optimizers on the clients ensure descent, the global updates will follow that for convex objectives. This result enables various line search techniques to be incorporated in our framework without losing their convergence guarantees in the federated setting. 

We presented the convergence rates for convex, strongly convex, and non-convex objectives. We showed that it achieves a linear rate for strongly convex objectives, which is available in only a couple of previous works. In particular, ours is the first work that guarantees linear convergence with partial participation for federated optimization of strongly convex objectives.  

Note that, for those schemes where descent is guaranteed, extra computation comes as an inherent character of the algorithm, which is then translated into the federated algorithm as well; this can be seen in our \flo algorithm. Nevertheless, the line-search schemes find a well-deserved place on the horizon of convex optimization methods, which was hitherto unexplored for federated optimization. Our work fills this gap.  



==> sections/model.tex <==
We consider a federated learning system with a \textit{server} and $N$ \textit{clients} that train a shared \textit{model} $w\in \mathbb{R}^d$. The training proceeds over $T$ number of \textit{synchronization rounds} take place, where a subset of clients $\mathcal{S}_t\subset [N]$ perform \textit{local} optimization at each synchronization round $t\in[T]$. For simplicity, we take $|\mathcal{S}_t|=S$ for all $t\in[T]$. On this system, we aim to solve the following optimization problem for the \textit{global objective} function $f$:
\begin{equation}\label{eqn:fm}
\min_{w\in \mathbb{R}^d} f(w):=\frac{1}{N}\sum_{i=1}^{N}f_i(w),
\end{equation}
where $f_i$ denotes the objective (loss) function of the $i$-th client for $i\in [N]$. 

At the beginning of the $t^{th}$ round, each participating client $i\in \mathcal{S}_t$ stores identical local copies of the model $w_{t,0}^i=w_t$ after communication time $t$ and performs $K$ local optimization steps, generally via iterative stochastic gradient-based scheme (\ref{eqn:clientlocal}), to update it to $w_{t,K}^i$ as the following iteration:
\begin{equation}\label{eqn:clientlocal}
w_{t,k+1}^i=w_{t,k}^i-\eta_{t,k}^ig_{t,k}^i,~\text{for}~k\in[K-1],
\end{equation}
where ${\eta_{t,k}^i}$ is the step-size for the $k$-th local step after $t$-th communication round and $g_{t,k}^i(w)$ is the stochastic gradient. Note that, the stochastic gradient $g_{t,k}^i(w)$ is an unbiased estimator of the gradient of local objective $\nabla f_i(w)$, i.e. $\mathbb{E}[g_{t,k}^i(w)]=\nabla f_i(w)$ for all $ t\in[T]$, $k\in[K]$ and $w\in \mathbb{R}^d$.

After performing $K$ local optimization steps, the updated model parameters of each client $w_{t,K}^i$ are used to compute the pseudo-gradient of the federated system as $\Delta_t:=\frac{1}{S}(w_t-w_{t,K}^i)$, that is essentially the the aggregated gradient across all rounds averaged for all participating clients.

%\subsection{\fli Algorithms}

\ignore{
	\Statex
	\Function{ClientUpdate}{$k, w$} \Comment{Run on client $k$}
	\State $B \leftarrow$ (split data at client $k$ into batches of size $B$)
	\For{each local epoch $i$ from $1$ to $E$}
	\For{batch $b \in B$}
	\If{\texttt{line\_search} == `DFW'} 
	\State $w_{t+1} \leftarrow \text{DFW}(w,b)$
	% \State $w_{t+1} \leftarrow w_t - \eta \mathcal{L} + \mathcal{D}$ % as comment Parameters update
	\ElsIf{\texttt{line\_search} == `armijo'}
	% \If{\texttt{line\_search} == 'armijo'}
	% \State $\eta \leftarrow 
	% \text{reset}(\eta, \eta_{\text{max}}, \gamma,b,t,opt)$
	\State $w_{t+1} \leftarrow \text{Armijo}(\text{f}, w_0, \eta_{\text{max}}, b, c, \beta, \gamma, \textit{opt})$
	% \State $w_{t+1} \leftarrow w_t$ 
	\Else
	\State $w_{t+1} \leftarrow w_t - \eta\nabla f_b(w_t)$
	
	% \Comment{Parameters update}
	
	
	\EndIf 
	\EndFor
	\EndFor
	\State \Return $w_{t+1}$ to server
	\EndFunction
	
	\subsection{Problem Formulation}
	We possess a dataset comprising N pairs, each consisting of a sample \( x_i \) in a \( d \)-dimensional space \( \mathbb{R}^d \), and an associated label \( y_i \) from a set of possible outcomes \( Y \). Within this framework, we employ a model characterized by a function \( f \) and a set of parameters \( w \) situated in a \( p \)-dimensional parameter space \( \mathbb{R}^p \). For any given input \( x_i \), the model is designed to output a prediction vector \( f(w, x_i) \) that spans the breadth of \( Y \), providing a score for each potential label.
	
	Central to our model's evaluation is a loss function \( L(s, y_i) \), where \( s \) is a vector in \( \mathbb{R}^{|Y|} \) representing the predicted scores across all labels. This loss function is critical, quantifying the discrepancy between the model's predictions and the actual ground truth label \( y_i \). By meticulously computing this risk, we can gauge the accuracy and reliability of our model's predictions, guiding us in refining and enhancing its performance. This setup provides a robust framework for navigating the complexities of predictive modelling, ensuring our approach is grounded in theory and applicable in practice. The loss we use is cross-entropy loss. For simplification we consider \( f(w)_i \) = \( f(w, x_i) \) and  \(L(s)_i\) = \( L(s, y_i) \)
	\[
	L_{CE} : (s, y) \in  \mathbb{R}^{|Y|} \times Y  = \log \left( \sum_{k \in Y} \exp(s_k) \right) - s_y
	\]
	
	\subsection{SGD Algorithm}
	In the SGD (Stochastic Gradient Descent) framework, the gradient of the objective function is evaluated concerning a single instance or a subset of instances, denoted by $i_k$, selected randomly from the training set during iteration $k$. The parameter update rule is given by 
	\[ w_{k+1} = w_k - \eta_k \nabla f_{i_k}(w_k), \]
	where $\eta_k$ signifies the learning rate and $\nabla f_{i_k}$ represents the gradient of the loss function for the chosen instance or subset. It is postulated that the stochastic gradient $\nabla f_{i_k}(w)$ provides an unbiased estimate, thus 
	\[ \mathbb{E}_i[\nabla f_i(w)] = \nabla f(w) \]
	for any parameter vector $w$. The Armijo line-search strategy is employed to adaptively adjust the learning rate $\eta_k$ at each step.
	
	\subsection{Armijo Line Search}
	The Armijo line search is a method that optimizes step size in stochastic settings by ensuring that the updated parameters decrease the loss function by a particular proportion, which is determined by a hyper-parameter named 'c.' This hyper-parameter scales the squared norm of the gradient. This technique is beneficial in deep learning because it involves minimal extra computation, typically just one additional forward pass per iteration. The Armijo line search starts with a maximum step size and reduces it until the condition is met. This often avoids the need for backtracking through effective step-size resetting strategies, thus maintaining robustness and performance across various settings. To select the step-size at iteration k, the condition for the Armijo line search is formalized as follows: \[ f_{i_k}(w_k - \eta_k \nabla f_{i_k}(w_k)) \leq f_{i_k}(w_k) - c \cdot \eta_k \|\nabla f_{i_k}(w_k)\|^2 \]
	Here,  $c > 0$ is a hyper-parameter and determines the extent of descent. This method, adapted for stochastic gradient descent, leverages function evaluations rather than gradient computations, making it computationally efficient, especially in deep learning contexts corresponding to additional forward passes.
	
	\subsection{Deep Franke Wolfe}
	DFW is designed for optimizing deep neural networks and adapts the Frank-Wolfe optimization method, traditionally used for linear models, to the complex structure of neural networks. The key feature of DFW is the computation of an optimal step-size \( \gamma_t \) within the range [0,1] for each iteration \( t \), which can be determined in closed-form, mainly when dealing with convex and piecewise linear loss functions.
	
	The computation of the step size \( \gamma_t \) and the update direction, which is the conditional gradient of the dual problem, allows for updates at the exact computational cost as standard Stochastic Gradient Descent (SGD). This is significant as it maintains the efficiency of SGD while potentially offering better optimization characteristics due to the optimal step-size calculation. The update rule for the DFW algorithm can be expressed as:
	
	\[ w_{t+1} = w_t - \eta \nabla \rho(w_t) + \gamma_t \nabla L_j(f_j(w_t)) \]
	
	where \( \eta \) is the learning rate, \( \rho \) is the regularization term, and \( L_j \) is the loss for the \( j \)-th sample.
	
	DFW's design ensures that only a single step is taken per proximal problem, avoiding over-solving an approximate problem and thereby speeding up convergence. The method's ability to automatically adjust the effective learning rate eliminates the need to manually design a learning rate schedule, which is a common challenge in SGD-based optimization. The paper confirms through experimental results that DFW often minimizes the learning objective faster than traditional SGD approaches.
}

